Probing Protoplanetary Disk Winds with C II Absorption

We present an analysis of wind absorption in the C II ${\lambda}1335$ doublet towards 40 classical T Tauri stars with archival far-ultraviolet (FUV) spectra obtained by the Hubble Space Telescope. Absorption features produced by fast or slow winds are commonly detected (36 out of 40 targets) in our sample. The wind velocity of the fast wind decreases with disk inclination, consistent with expectations for a collimated jet. Slow wind absorption is detected mostly in disks with intermediate or high inclination, without a significant dependence of wind velocity on disk inclination. Both the fast and slow wind absorption are preferentially detected in FUV lines of neutral or singly ionized atoms. The Mg II ${\lambda}{\lambda}2796,2804$ lines show wind absorption consistent with the absorption in the C II lines. We develop simplified semi-analytical disk/wind models to interpret the observational disk wind absorption. Both fast and slow winds are consistent with expectations from a thermal-magnetized disk wind model and are generally inconsistent with a purely thermal wind. Both the models and the observational analysis indicate that wind absorption occurs preferentially from the inner disk, offering a wind diagnostic in complement to optical forbidden line emission that traces the wind in larger volumes.

==> Probing Disk Wind with Absorption Lines_astro-ph/figset.tex <==
\figsetstart
\figsetnum{6}
\figsettitle{UV Line Profiles}

\figsetgrpstart
\figsetgrpnum{6.1}
\figsetgrptitle{AA Tau}
\figsetplot{Figures/figset/AATau2013_ionization.pdf}
\figsetgrpnote{AA Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.2}
\figsetgrptitle{AK Sco}
\figsetplot{Figures/figset/AKSco_ionization.pdf}
\figsetgrpnote{AK Sco - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.3}
\figsetgrptitle{BP Tau}
\figsetplot{Figures/figset/BPTau_ionization.pdf}
\figsetgrpnote{BP Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.4}
\figsetgrptitle{CS Cha}
\figsetplot{Figures/figset/CSCha_ionization.pdf}
\figsetgrpnote{CS Cha - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.5}
\figsetgrptitle{CV Cha}
\figsetplot{Figures/figset/CVCha_ionization.pdf}
\figsetgrpnote{CV Cha - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.6}
\figsetgrptitle{CW Tau}
\figsetplot{Figures/figset/CWTau_ionization.pdf}
\figsetgrpnote{CW Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.7}
\figsetgrptitle{CY Tau}
\figsetplot{Figures/figset/CYTau_ionization.pdf}
\figsetgrpnote{CY Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.8}
\figsetgrptitle{DE Tau}
\figsetplot{Figures/figset/DETau_ionization.pdf}
\figsetgrpnote{DE Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.9}
\figsetgrptitle{DF Tau}
\figsetplot{Figures/figset/DFTau_ionization.pdf}
\figsetgrpnote{DF Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.10}
\figsetgrptitle{DK Tau}
\figsetplot{Figures/figset/DKTau_ionization.pdf}
\figsetgrpnote{DK Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.11}
\figsetgrptitle{DM Tau}
\figsetplot{Figures/figset/DMTau_ionization.pdf}
\figsetgrpnote{DM Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.12}
\figsetgrptitle{DN Tau}
\figsetplot{Figures/figset/DNTau_ionization.pdf}
\figsetgrpnote{DN Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.13}
\figsetgrptitle{DR Tau}
\figsetplot{Figures/figset/DRTau_ionization.pdf}
\figsetgrpnote{DR Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.14}
\figsetgrptitle{DS Tau}
\figsetplot{Figures/figset/DSTau_ionization.pdf}
\figsetgrpnote{DS Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.15}
\figsetgrptitle{GM Aur}
\figsetplot{Figures/figset/GMAur_ionization.pdf}
\figsetgrpnote{GM Aur - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.16}
\figsetgrptitle{HD 104237}
\figsetplot{Figures/figset/HD104237_ionization.pdf}
\figsetgrpnote{HD 104237 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.17}
\figsetgrptitle{HD 135344b}
\figsetplot{Figures/figset/HD135344b_ionization.pdf}
\figsetgrpnote{HD 135344b - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.18}
\figsetgrptitle{HD 142527}
\figsetplot{Figures/figset/HD142527_ionization.pdf}
\figsetgrpnote{HD 142527 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.19}
\figsetgrptitle{HD 169142}
\figsetplot{Figures/figset/HD169142_ionization.pdf}
\figsetgrpnote{HD 169142 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.20}
\figsetgrptitle{HN Tau}
\figsetplot{Figures/figset/HNTau_ionization.pdf}
\figsetgrpnote{HN Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.21}
\figsetgrptitle{IP Tau}
\figsetplot{Figures/figset/IPTau_ionization.pdf}
\figsetgrpnote{IP Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.22}
\figsetgrptitle{KK Oph}
\figsetplot{Figures/figset/KKOph_ionization.pdf}
\figsetgrpnote{KK Oph - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.23}
\figsetgrptitle{LkCa 15}
\figsetplot{Figures/figset/LkCa15_ionization.pdf}
\figsetgrpnote{LkCa 15 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.24}
\figsetgrptitle{PDS 66}
\figsetplot{Figures/figset/PDS66_ionization.pdf}
\figsetgrpnote{PDS 66 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.25}
\figsetgrptitle{RECX 11}
\figsetplot{Figures/figset/RECX11_ionization.pdf}
\figsetgrpnote{RECX 11 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.26}
\figsetgrptitle{RECX 15}
\figsetplot{Figures/figset/RECX15_2010_ionization.pdf}
\figsetgrpnote{RECX 15 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.27}
\figsetgrptitle{RR Tau}
\figsetplot{Figures/figset/RRTau_ionization.pdf}
\figsetgrpnote{RR Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.28}
\figsetgrptitle{RU Lup}
\figsetplot{Figures/figset/RULup_ionization.pdf}
\figsetgrpnote{RU Lup - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.29}
\figsetgrptitle{RW Aur}
\figsetplot{Figures/figset/RWAur2013_ionization.pdf}
\figsetgrpnote{RW Aur - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.30}
\figsetgrptitle{RY Lup}
\figsetplot{Figures/figset/RYLup_ionization.pdf}
\figsetgrpnote{RY Lup - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.31}
\figsetgrptitle{SU Aur}
\figsetplot{Figures/figset/SUAur_ionization.pdf}
\figsetgrpnote{SU Aur - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.32}
\figsetgrptitle{SZ 68}
\figsetplot{Figures/figset/SZ68_ionization.pdf}
\figsetgrpnote{SZ 68 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.33}
\figsetgrptitle{T Cha}
\figsetplot{Figures/figset/TCha_ionization.pdf}
\figsetgrpnote{T Cha - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.34}
\figsetgrptitle{T Ori}
\figsetplot{Figures/figset/TOri_ionization.pdf}
\figsetgrpnote{T Ori - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.35}
\figsetgrptitle{T Tau}
\figsetplot{Figures/figset/TTau_ionization.pdf}
\figsetgrpnote{T Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.36}
\figsetgrptitle{TW Hya}
\figsetplot{Figures/figset/TWHya_ionization.pdf}
\figsetgrpnote{TW Hya - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.37}
\figsetgrptitle{UX Tau}
\figsetplot{Figures/figset/UXTau_ionization.pdf}
\figsetgrpnote{UX Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.38}
\figsetgrptitle{V836 Tau}
\figsetplot{Figures/figset/V836Tau_ionization.pdf}
\figsetgrpnote{V836 Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.39}
\figsetgrptitle{V4046 Sgr}
\figsetplot{Figures/figset/V4046Sgr_ionization.pdf}
\figsetgrpnote{V4046 Sgr - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.40}
\figsetgrptitle{VV Ser}
\figsetplot{Figures/figset/VVSer_ionization.pdf}
\figsetgrpnote{VV Ser - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetend

==> figset.tex <==
\figsetstart
\figsetnum{6}
\figsettitle{UV Line Profiles}

\figsetgrpstart
\figsetgrpnum{6.1}
\figsetgrptitle{AA Tau}
\figsetplot{Figures/figset/AATau2013_ionization.pdf}
\figsetgrpnote{AA Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.2}
\figsetgrptitle{AK Sco}
\figsetplot{Figures/figset/AKSco_ionization.pdf}
\figsetgrpnote{AK Sco - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.3}
\figsetgrptitle{BP Tau}
\figsetplot{Figures/figset/BPTau_ionization.pdf}
\figsetgrpnote{BP Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.4}
\figsetgrptitle{CS Cha}
\figsetplot{Figures/figset/CSCha_ionization.pdf}
\figsetgrpnote{CS Cha - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.5}
\figsetgrptitle{CV Cha}
\figsetplot{Figures/figset/CVCha_ionization.pdf}
\figsetgrpnote{CV Cha - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.6}
\figsetgrptitle{CW Tau}
\figsetplot{Figures/figset/CWTau_ionization.pdf}
\figsetgrpnote{CW Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.7}
\figsetgrptitle{CY Tau}
\figsetplot{Figures/figset/CYTau_ionization.pdf}
\figsetgrpnote{CY Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.8}
\figsetgrptitle{DE Tau}
\figsetplot{Figures/figset/DETau_ionization.pdf}
\figsetgrpnote{DE Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.9}
\figsetgrptitle{DF Tau}
\figsetplot{Figures/figset/DFTau_ionization.pdf}
\figsetgrpnote{DF Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.10}
\figsetgrptitle{DK Tau}
\figsetplot{Figures/figset/DKTau_ionization.pdf}
\figsetgrpnote{DK Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.11}
\figsetgrptitle{DM Tau}
\figsetplot{Figures/figset/DMTau_ionization.pdf}
\figsetgrpnote{DM Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.12}
\figsetgrptitle{DN Tau}
\figsetplot{Figures/figset/DNTau_ionization.pdf}
\figsetgrpnote{DN Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.13}
\figsetgrptitle{DR Tau}
\figsetplot{Figures/figset/DRTau_ionization.pdf}
\figsetgrpnote{DR Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.14}
\figsetgrptitle{DS Tau}
\figsetplot{Figures/figset/DSTau_ionization.pdf}
\figsetgrpnote{DS Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.15}
\figsetgrptitle{GM Aur}
\figsetplot{Figures/figset/GMAur_ionization.pdf}
\figsetgrpnote{GM Aur - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.16}
\figsetgrptitle{HD 104237}
\figsetplot{Figures/figset/HD104237_ionization.pdf}
\figsetgrpnote{HD 104237 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.17}
\figsetgrptitle{HD 135344b}
\figsetplot{Figures/figset/HD135344b_ionization.pdf}
\figsetgrpnote{HD 135344b - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.18}
\figsetgrptitle{HD 142527}
\figsetplot{Figures/figset/HD142527_ionization.pdf}
\figsetgrpnote{HD 142527 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.19}
\figsetgrptitle{HD 169142}
\figsetplot{Figures/figset/HD169142_ionization.pdf}
\figsetgrpnote{HD 169142 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.20}
\figsetgrptitle{HN Tau}
\figsetplot{Figures/figset/HNTau_ionization.pdf}
\figsetgrpnote{HN Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.21}
\figsetgrptitle{IP Tau}
\figsetplot{Figures/figset/IPTau_ionization.pdf}
\figsetgrpnote{IP Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.22}
\figsetgrptitle{KK Oph}
\figsetplot{Figures/figset/KKOph_ionization.pdf}
\figsetgrpnote{KK Oph - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.23}
\figsetgrptitle{LkCa 15}
\figsetplot{Figures/figset/LkCa15_ionization.pdf}
\figsetgrpnote{LkCa 15 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.24}
\figsetgrptitle{PDS 66}
\figsetplot{Figures/figset/PDS66_ionization.pdf}
\figsetgrpnote{PDS 66 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.25}
\figsetgrptitle{RECX 11}
\figsetplot{Figures/figset/RECX11_ionization.pdf}
\figsetgrpnote{RECX 11 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.26}
\figsetgrptitle{RECX 15}
\figsetplot{Figures/figset/RECX15_2010_ionization.pdf}
\figsetgrpnote{RECX 15 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.27}
\figsetgrptitle{RR Tau}
\figsetplot{Figures/figset/RRTau_ionization.pdf}
\figsetgrpnote{RR Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.28}
\figsetgrptitle{RU Lup}
\figsetplot{Figures/figset/RULup_ionization.pdf}
\figsetgrpnote{RU Lup - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.29}
\figsetgrptitle{RW Aur}
\figsetplot{Figures/figset/RWAur2013_ionization.pdf}
\figsetgrpnote{RW Aur - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.30}
\figsetgrptitle{RY Lup}
\figsetplot{Figures/figset/RYLup_ionization.pdf}
\figsetgrpnote{RY Lup - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.31}
\figsetgrptitle{SU Aur}
\figsetplot{Figures/figset/SUAur_ionization.pdf}
\figsetgrpnote{SU Aur - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.32}
\figsetgrptitle{SZ 68}
\figsetplot{Figures/figset/SZ68_ionization.pdf}
\figsetgrpnote{SZ 68 - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.33}
\figsetgrptitle{T Cha}
\figsetplot{Figures/figset/TCha_ionization.pdf}
\figsetgrpnote{T Cha - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.34}
\figsetgrptitle{T Ori}
\figsetplot{Figures/figset/TOri_ionization.pdf}
\figsetgrpnote{T Ori - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.35}
\figsetgrptitle{T Tau}
\figsetplot{Figures/figset/TTau_ionization.pdf}
\figsetgrpnote{T Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.36}
\figsetgrptitle{TW Hya}
\figsetplot{Figures/figset/TWHya_ionization.pdf}
\figsetgrpnote{TW Hya - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.37}
\figsetgrptitle{UX Tau}
\figsetplot{Figures/figset/UXTau_ionization.pdf}
\figsetgrpnote{UX Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.38}
\figsetgrptitle{V836 Tau}
\figsetplot{Figures/figset/V836Tau_ionization.pdf}
\figsetgrpnote{V836 Tau - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.39}
\figsetgrptitle{V4046 Sgr}
\figsetplot{Figures/figset/V4046Sgr_ionization.pdf}
\figsetgrpnote{V4046 Sgr - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{6.40}
\figsetgrptitle{VV Ser}
\figsetplot{Figures/figset/VVSer_ionization.pdf}
\figsetgrpnote{VV Ser - FUV line profiles of different ionization states and Mg II NUV line profiles, if present. Dashed horizontal lines mark the zero-flux level for each line. The dashed vertical line shows zero-velocity.}
\figsetgrpend

\figsetend
